Extending the OpenCHK Model with Advanced Checkpoint Features

One of the major challenges in using extreme scale systems efficiently is to mitigate the impact of faults. Application-level checkpoint/restart (CR) methods provide the best trade-off between productivity, robustness, and performance. There are many solutions implementing CR at the application level. They all provide advanced I/O capabilities to minimize the overhead introduced by CR. Nevertheless, there is still room for improvement in terms of programmability and flexibility, because end-users must manually serialize and deserialize application state using low-level APIs, modify the flow of the application to consider restarts, or rewrite CR code whenever the backend library changes. In this work, we propose a set of compiler directives and clauses that allow users to specify CR operations in a simple way. Our approach supports the common CR features provided by all the CR libraries. However, it can also be extended to support advanced features that are only available in some CR libraries, such as differential checkpointing, the use of HDF5 format, and the possibility of using fault-tolerance-dedicated threads. The result of our evaluation revealed a high increase in programmability. On average, we reduced the number of lines of code by 71%, 94%, and 64% for FTI, SCR, and VeloC, respectively, and no additional overhead was perceived using our solution compared to using the backend libraries directly. Finally, portability is enhanced because our programming model allows the use of any backend library without changing any code.

==> Makefile <==
#
# $Id: Makefile 279 2008-01-27 16:19:38Z balaji $
#
# Copyright (C) 2006-2007, University of Chicago. All rights reserved.
#

HEADER = tcl_all
REVIEWS = responseToReviewers
PICS = figures
BIB = bib
#TEX = text
EXAMPLES = examples
PDFLATEX = pdflatex

TARGETS: $(HEADER).pdf $(REVIEWS).pdf
.PHONY: all clean

example_files = $(shell find $(EXAMPLES) -name '*.tex' -print)
tex_files = $(shell find $(TEX) -name '*.tex' -print)
bib_files = $(shell find $(BIB) -name '*.bib' -print)
pic_files = $(shell find $(PICS) \
		\( -name '*.eps' -print \) -or \( -name '*.epsi' -print \) \
		-or \( -name '*.ps' -print \) -or \( -name '*.png' -print \) \
		-or \( -name '*.fig' -print \) -or \( -name '*.pdf' -print \) \
		-or \( -name '*.jpg' -print \) -or \( -name '*.jpeg' -print \) \
	)

$(REVIEWS).pdf: $(REVIEWS).tex
	$(PDFLATEX) $(REVIEWS)	

$(HEADER).pdf: $(HEADER).tex $(tex_files) $(example_files) $(bib_files) $(pic_files)
	@if test "`which rubber`" != "" ; then \
		TEXMFOUTPUT=`pwd` rubber -d $(HEADER); \
	else \
		$(PDFLATEX) $(HEADER) | tee latex.out ; \
		if grep -q '^LaTeX Warning: Citation.*undefined' latex.out; then \
			bibtex $(HEADER); \
			touch .rebuild; \
		fi ; \
		while [ -f .rebuild -o \
			-n "`grep '^LaTeX Warning:.*Rerun' latex.out`" ]; do \
			rm -f .rebuild; \
			$(PDFLATEX) $(HEADER) | tee latex.out; \
		done ; \
		rm -f latex.out ; \
	fi
#	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dNOPAUSE -dQUIET -dBATCH -sOutputFile=$(HEADER)-compressed.pdf $(HEADER).pdf
#	mv $(HEADER)-compressed.pdf $(HEADER).pdf

debug:
	@echo $(HEADER).tex $(tex_files) $(bib_files) $(pic_files)

clean-pdf:
	rm $(HEADER).pdf $(REVIEWS).pdf
clean:
	@if test "`which rubber`" != "" ; then \
		rubber -d --clean $(HEADER) ; \
	else \
		find . \( -name '*.blg' -print \) -or \( -name '*.aux' -print \) -or \
			\( -name '*.bbl' -print \) -or \( -name '*~' -print \) -or \
			\( -name '*.lof' -print \) -or \( -name '*.lot' -print \) -or \
			\( -name '*.toc' -print \) | xargs rm -f; \
		rm -f $(HEADER).dvi $(HEADER).log $(HEADER).ps $(HEADER).pdf $(HEADER).out \
			_region_* TAGS ; \
	fi

